GPTAraEval: A Comprehensive Evaluation of ChatGPT on Arabic NLP

ChatGPT's emergence heralds a transformative phase in NLP, particularly demonstrated through its excellent performance on many English benchmarks. However, the model's efficacy across diverse linguistic contexts remains largely uncharted territory. This work aims to bridge this knowledge gap, with a primary focus on assessing ChatGPT's capabilities on Arabic languages and dialectal varieties. Our comprehensive study conducts a large-scale automated and human evaluation of ChatGPT, encompassing 44 distinct language understanding and generation tasks on over 60 different datasets. To our knowledge, this marks the first extensive performance analysis of ChatGPT's deployment in Arabic NLP. Our findings indicate that, despite its remarkable performance in English, ChatGPT is consistently surpassed by smaller models that have undergone finetuning on Arabic. We further undertake a meticulous comparison of ChatGPT and GPT-4's Modern Standard Arabic (MSA) and Dialectal Arabic (DA), unveiling the relative shortcomings of both models in handling Arabic dialects compared to MSA. Although we further explore and confirm the utility of employing GPT-4 as a potential alternative for human evaluation, our work adds to a growing body of research underscoring the limitations of ChatGPT.

==> PREV/PREV_msa_vs_da.tex <==
\section{MSA \textit{vs} DA}

\textbf{How does ChatGPT perform on MSA \textit{vs} DA?} We investigate how ChatGPT perform on modern standard Arabic (MSA) and Dialectical Arabic (DA). For this purpose, we first select DA tasks from ORCA. We then run an in-house strong MSA \textit{vs} DA classifier to separate MSA and DA samples. We only select those samples on which the classifier is atleast $80$\% confidence during the prediction. We then evaluate the macro-F\textsubscript{1} performance of ChatGPT on the selected samples.


%%%%%%%%%%%%%%%%%%%%%%%%%  Figure %%%%%%%%%%%%%%%%%

\begin{figure*}[h]
\centering
  \includegraphics[height = 0.5\textwidth]{Figures/msa_da_orca.png}
  \caption{MSA \textit{vs} DA performance (macro-F\textsubscript{1}) comparison of ChatGPT on $11$ ORCA tasks.}
  \label{fig:msa_da_orca}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent As shown in Figure~\ref{fig:msa_da_orca}, ChatGPT performs well on MSA samples compared to DA samples on the majority ($8$ out of $11$) of the tasks. \textit{This result shows that ChatGPT has seen more MSA data than DA during its pretraining.}


\noindent \textbf{How does ChatGPT perform on different dialects?} To further probe the impact of ChatGPT on different Arabic dialect, we evaluate ChatGPT on MSA and five Arabic Dialects $\rightarrow$ English machine translation tasks using the Multi-dialectal Parallel Corpus (MDPC) proposed by~\newcite{bouamor2014multidialectal}.

%%%%%%%%%%%%%%%%%%%%%%%%%  Figure %%%%%%%%%%%%%%%%%

\begin{figure}[h]
  \includegraphics[height = 0.7\linewidth]{Figures/dt_chatgpt.png}
  \caption{BLEU scores of ChatGPT on MSA and five Arabic Dialects $\rightarrow$ English machine translation tasks for few-shot settings.}
  \label{fig:dt_chatgpt}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We show BLEU score of ChatGPT on MT tasks for MSA and five dialects in Figure~\ref{fig:dt_chatgpt}. As expected, ChatGPT MSA performance outperforms dialectal performance on all the shots, which further substantiate our previous hypothesis. In comparison among the dialects, ChatGPT performs best on \textit{Egyptian} dialect. We postulate that this is also directly correlated with the availability of the dialectal data. For example, the quantity of \textit{Egyptian} open-sourced pretraining data is more than any other dialect available online~\citep{nagoudi2022jasmine}. On the other hand, ChatGPT exhibits better performance on \textit{Jordanian} dialect than the rests. We suspect the reason is due to high overlap of \textit{Jordanian} dialect with MSA~\citep{bouamor2014multidialectal}. The other dialects, namely, \textit{Palestinian}, \textit{Syrian}, and \textit{Tunisian} dialects perform very close to each other but underperform compared to \textit{Egyptian} and \textit{Jordanian} dialects.


\noindent \textbf{How does ChatGPT perform compared to GPT4?} We conduct comparative performance analysis between ChatGPT and GPT4 on the dialectal machine translation tasks. Specifically, we would like to investigate whether GPT4 can improve over ChatGPT for dialects (\textit{Palestinian}, \textit{Syrian}, and \textit{Tunisian}) situated in the lower spectrum of the ChatGPT's performance. To experiment with GPT4, we randomly sample $50$ examples from MSA and dialectal translation datasets, then generate response with GPT4. We select the same $50$ examples for ChatGPT generation to make fair comparison. We then compare BLEU scores of ChatGPT and GPT4 responses.


%%%%%%%%%%%%%%%%%%%%%%%%%  Figure %%%%%%%%%%%%%%%%%

\begin{figure}[h]
  \includegraphics[height = 0.7\linewidth]{Figures/dt_chatgpt_gpt4.png}
  \caption{Performance (BLEU) comparison between ChatGPT and GPT4 on MSA and five Arabic Dialects $\rightarrow$ English machine translation tasks for $0$- and $3$-shot settings.}
  \label{fig:dt_chatgpt_gpt4}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent Figure~\ref{fig:dt_chatgpt_gpt4} shows the performance comparison between ChatGPT and GPT4 with $0$- and $3$-shot settings. We observe that GPT4 outperforms ChatGPT on MSA with $0$-shot but ChatGPT outperforms GPT4 with $3$-shot learning. On \textit{Egyptian} dialect, ChatGPT outperforms GPT4, whereas on \textit{Jordanian} dialect, GPT4 outperforms ChatGPT. Notably, on the dialects (\textit{Palestinian}, \textit{Syrian}, and \textit{Tunisian}) where ChatGPT struggles to perform comparatively well, GPT4 improves over ChatGPT (with an exception to $3$-shot learning on \textit{Syrian} dialect). This finding shows that ChatGPT can perform on par or even better than GPT4 with sufficiently available dialectal data (e.g., \textit{Egyptian}), while GPT4 can improve over ChatGPT on comparatively low-resourced dialects.

==> acw.tex <==
% \section{Analysis and Discussion}\label{sec:disc}

\section*{Acknowledgements}\label{sec:acknow}
% We gratefully acknowledge support from the Natural Sciences and Engineering Research Council of Canada (NSERC; RGPIN-2018-04267), the Social Sciences and Humanities Research Council of Canada (SSHRC; 435-2018-0576; 895-2020-1004; 895-2021-1008), Canadian Foundation for Innovation (CFI; 37771), Compute Canada (CC), and \footnote{\href{https://www.computecanada.ca}{https://www.computecanada.ca}} UBC ARC-Sockeye,\footnote{\href{https://arc.ubc.ca/ubc-arc-sockeye}{https://arc.ubc.ca/ubc-arc-sockeye}}. Any opinions, conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of NSERC, SSHRC, CFI, CC, AMD, or UBC ARC-Sockeye. 

% {Acknowledgements}\label{sec:acknow}
We gratefully acknowledge support from Canada Research Chairs (CRC), the Natural Sciences and Engineering Research Council of Canada (NSERC; RGPIN-2018-04267), the Social Sciences and Humanities Research Council of Canada (SSHRC; 435-2018-0576; 895-2020-1004; 895-2021-1008), Canadian Foundation for Innovation (CFI; 37771), Digital Research Alliance of Canada,\footnote{\href{https://alliancecan.ca}{https://alliancecan.ca}} UBC ARC-Sockeye,\footnote{\href{https://arc.ubc.ca/ubc-arc-sockeye}{https://arc.ubc.ca/ubc-arc-sockeye}} and Google TPU Research Cloud (TRC).\footnote{\href{https://sites.research.google/trc/about/}{https://sites.research.google/trc/about/}} Any opinions, conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of CRC, NSERC, SSHRC, CFI, DRAG, Google, or UBC ARC-Sockeye.

==> da_country_nlu.tex <==
\section{Performance of \ChatGPT on Country-wise NLU}
In addition to evaluating \ChatGPT on MSA \textit{vs} DA language understanding tasks (Section~\ref{sec:msa_da}), we assess \ChatGPT on country-level dialectal understanding. For this purpose, we first select DA tasks from ORCA. We then run the MSA \textit{vs} DA classifier to separate MSA and DA samples. Upon selecting only the DA samples, we ran an in-house strong country-level dialect detection classifier. We only select those samples on which the classifier is at least $50$\% confident during the prediction. We then evaluate the macro-F\textsubscript{1} performance of \ChatGPT selected samples.


%%%%%%%%%%%%%%%%%%%%%%%%%  Table %%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccccccccccccc}
\hline
Country & Algeria & Libya & UAE   & Egypt & Yemen & Saudi Arabia & Syria & Tunisia & Palestine & Jordan & Qatar & Lebanon & Kuwait & Bahrain & Sudan & Iraq  & Oman  & Morocco \\ \hline
Macro F\textsubscript{1}      & 39.29   & 37.95 & 31.67 & 31.61 & 31.44 & 31.14        & 31.10 & 30.51   & 29.46     & 29.30  & 24.17 & 23.43   & 22.93  & 22.78   & 21.94 & 19.84 & 19.17 & 12.78   \\ \hline
\end{tabular}
}
\caption{
\label{tab:da_country}
Performance of \ChatGPT on \textit{country}-wise NLU tasks.
}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We present the result in Table~\ref{tab:da_country}. As evident, \ChatGPT performs best on the samples coming from Algeria, Libya, UAE, Egypt. On the other hand, \ChatGPT shows inferior performance on the samples coming from Iraq, Oman, Morocco.

==> discussion.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%  Figure %%%%%%%%%%%%%%%%%

\begin{figure*}[h]
  \includegraphics[width = \linewidth]{Figures/dataset_cleaning.pdf}
  \caption{Prediction samples of ChatGPT on the age and the gender detection tasks. ChatGPT correctly identifies insufficient context in the datasets.}
  \label{fig:dataset_cleaning}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Discussion}
\label{sec:discussion}



%As a result of this limitation, ChatGPT may often flag non-harmful prompts as toxic. We believe such behavior of ChatGPT can hinder generating diversified multilingual texts, especially in Arabic.


\noindent \textbf{\ChatGPT can be utilized for identifying weak training samples.} We notice that performance of both \AraTF and \ChatGPT very low on the demographic tasks (Table~\ref{tab:nlu-results}). We perform an error analysis on all data misclassified by \ChatGPT, finding that \ChatGPT refuses to predict labels for samples with weak demographic cues (for age and gender prediction). That is, \ChatGPT outputs a message explicitly stating that input text has insufficient context for predicting labels (Figure~\ref{fig:dataset_cleaning}). 
Our human analysis shows that these sample do lack sufficient cues for these tasks. As such, we believe \ChatGPT can be used to identify weak training samples.



%We find that some examples in these datasets are indeed lack in providing sufficient information to classify the with correct labels. Such presence of outliers which do not provide enough context are inevitable, considering that these datasets are collected from Twitter with weak supervision~\citep{orca}. However, this finding shows that we can leverage ChatGPT for detecting weak examples, especially when human supervision deems costly for large amount of data.


%%%%%%%%%%%%%%%%%%%%%%%%%  Figure %%%%%%%%%%%%%%%%%

\begin{figure}[h]
  \includegraphics[height = 0.7\linewidth]{Figures/cm_xnli.png}
  \caption{Confusion Matrix on the XNLI tasks. ChatGPT prones to misclassify neutral examples.}
  \label{fig:cm_xnli}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{ChatGPT excels at binary text-pair inference.} As shown in Table~\ref{tab:nlu-results}, ChatGPT achieves close (stance detection) or even higher (paraphrase detection) performance compared to the finetuned AraT5 models on the text-pair classification tasks (which are both binary classification tasks). Meanwhile, ChatGPT performs poorly compared to the finetuned model on the multiclass XNLI Arabic dataset. Upon inspection, we find that ChatGPT cannot confidently detect the \textit{neutral} class of XNLI (see Figure~\ref{fig:cm_xnli}). This may suggest that ChatGPT, similar to many text classification models, performs better on binary classification tasks with clear separation than on multiclass tasks that require more nuanced language understanding. Further, these results suggest that ChatGPT excels on semantics-level tasks such as paraphrase detection even in languages such as Arabic.

%It is to be noted that both paraphrase and stance detection are two-class classification tasks, whereas XNLI is a three-class classification task. Therefore, we resort to find out which class in XNLI is mostly responsible for the poor performance. As evident in Figure~\ref{fig:cm_xnli}, ChatGPT mostly misclassifies neutral examples. We conjecture that the model has seen more binary inference tasks like paraphrase detection or stance detection against slightly more complex datasets with multiclass labels for inference. As a result, the model overfits on those opposite classes (entailment, contradiction) and wrongly predicts neutral examples into those classes.



\begin{comment}

\subsection{Why BLOOMZ Outperforms ChatGPT on Some NLG Tasks}

Unlike the performance on the NLU tasks (Section~\ref{sec:eval_nlu}) where ChatGPT completely dominates BLOOMZ, we observe that BLOOMZ being a smaller model, performs better than ChatGPT on some of the NLG tasks (Section~\ref{sec:eval_nlg}). Especially, we can see, BLOOMZ outperforms ChatGPT on question generation and answering, style transfer, and paraphrase generation tasks. To investigate the rationale behind this, we find that BLOOMZ is finetuned on some of the evaluation tasks. For example, multilingual question-answering datasets like MLQA~\citep{lewis2019mlqa} and xQuAD~\citep{artetxe2020cross} are used to finetune BLOOMZ, while dataset like PAWS-X~\citep{pawsx} is used to finetune BLOOMZ on the multilingual paraphasing tasks. Therefore, when we evaluate the models on similar Arabic NLG tasks, BLOOMZ can leverage advantage over ChatGPT.
    
\end{comment}

==> human-evaluation-table-concise.tex <==
\begin{table}[h!]
\resizebox{0.46\textwidth}{!}{
\begin{tabular}{lccc}
\hline
Task     & \begin{tabular}[c]{@{}c@{}}\ChatGPT\\ (A/B/C/D)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\BLOOMZ\\ (A/B/C/D)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\GPTF\\ (A/B/C/D)\end{tabular} \\ \hline

Paraph   & 87/9/04     & 6/2/3/89    & 84/7/2/7   \\
Summ     & 85/10/6/0   & 26/12/35/27 & 91/9/0/0   \\
MSA\_Fr* & 55/26/4/15  & 5/9/8/78    & 88/11/1/0  \\
Jor\_En* & 58/26/13/3  & 9/9/10/72   & 75/18/5/2  \\
Fr\_Ar   & 74/25/1/0   & 8/30/15/47  & 63/36/1/0  \\
DG\_Egy  & 41/24/29/6  & 0/0/0/100   & 42/31/8/19 \\
DG\_Lev  & 23/16/49/12 & 1/0/0/99    & 65/19/10/6 \\
DG\_Lev  & 26/9/58/7   & 0/0/0/100   & 32/22/42/4 \\ \hline
\end{tabular}}
\caption{\label{tab:human-evaluation-concise}
Human evaluation results are aggregated from two annotators. 50 examples per task. A, B, C D (/ separated) indicates the rating from each model. A is the best, and D is the worst possible rating. * indicates Code-Switched Machine Translation task. DG stands for Dialogue Generation. 
}
\end{table}

==> human_cst.tex <==
\section{Human Analysis on CST}

As evident from Table~\ref{tab:nlg-results}, \ChatGPT outperforms the finetuned model on the code-switched translation task. This prompted us to further probe \ChatGPT’s code-switching ability using diagnostic test cases. Specifically, we manually evaluated \ChatGPT’s capability of English mixed MSA, Egyptian, and Moroccan code-switched translation generation from plain English text. We ask two annotators who are fluent on the respective varieties (as well as English), to evaluate a the diagnostic dataset based on \textit{fluency} (defined as how fluent the translated text is), \textit{faithfulness} (defined as how semantically close the translated text is to the source text), and \textit{code-switching ability} (defined as how accurately the translated text includes the code-switch scripts). We present our result in the Table~\ref{tab:human_cst}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\footnotesize 
\renewcommand*{\arraystretch}{0.8}   %to squeeze table content
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{ccccc}
{\textbf{Annotator}} & {\textbf{CST}}             & {\textbf{fluency (A/B/C/D)}} & {\textbf{faithfulness (A/B/C/D)}} & {\textbf{code-switching (A/B/C/D)}} \\
{Annotator 1}        & {En \rightarrow MSA-En} & {80/10/10/0}                 & {80/20/0/0}                       & {0/40/0/60}                         \\
{}                   & {En \rightarrow Egy-En} & {70/10/20/0}                 & {100/0/0/0}                       & {20/30/0/50}                        \\
{}                   & {En \rightarrow Mor-En} & {10/40/50/0}                 & {90/0/10/0}                       & {20/30/0/50}                        \\
{}                   & {\textit{\textbf{Avg}}}    & {53.3/20/26.7/0}             & {90/6.7/3.3/0}                    & {13.3/33.3/0/53.4}                  \\
{Annotator 2}        & {En \rightarrow MSA-En} & {30/70/0/0}                  & {90/0/10/0}                       & {0/30/0/70}                         \\
{}                   & {En \rightarrow Egy-En} & {50/40/10/0}                 & {90/10/0/0}                       & {0/40/0/60}                         \\
{}                   & {En \rightarrow Mor-En} & {20/40/40/0}                 & {100/0/0/0}                       & {20/30/0/50}                        \\
{}                   & {\textit{\textbf{Avg}}}    & {33.3/50/16.7}               & {93.4/3.3/3.3/0}                  & {6.7/33.3/0/60}                     \\
{\textbf{Average}}   & {\textit{\textbf{}}}       & {43.3/35/21.7/0}             & {91.7/5/3.3/0}                    & {10/33.3/0/56.7}                   
\end{tabular}
}
\caption{
\label{tab:human_cst}
Human evaluation of \ChatGPT's responses on the three code-switched translation tasks.
}

\end{table}

From Table~\ref{tab:human_cst}, we observe that \ChatGPT produces fluent translations that are also semantically close (faithful) to the source text. However, \ChatGPT struggles to produce code-switched text and generates mostly in Arabic script. Interestingly, this issue is more prevalent for MSA than Egyptian and Moroccan. We hypothesize that the tokens in the source English text are very common in MSA. As a result, the model does not seem \textit{willing} to code-switch the words into English.
